Higher-Curvature Gravity and Entanglement Entropy

In this thesis, we focus on higher-curvature extensions of Einstein gravity as toy models to probe universal properties of conformal field theory (CFT) using the gauge/gravity duality. In this context, we are particularly interested in generalized quasi-topological gravities, i.e., theories whose equations of motion for statically spherically symmetric solutions are of second order at most. Here, we characterize the number of these theories existing at a given curvature order and dimensions. Moreover, we show that any effective higher-curvature theory is connected, via field redefinitions to some generalized quasi-topological gravity. The situation is special for three spacetime dimensions, as theories of this type have trivial equations of motion. However, when matter fields are added into the picture, the equations of motion become non-trivial, describing, among other solutions, multiparametric generalizations of the Ba\~nados-Teitelboim-Zanelli black hole. From the CFT side, entanglement entropy arises as a prominent quantity that encodes important information about the field theory, such as the type A and type B trace anomalies in even dimensions and the sphere free energy of the theory in odd dimensions when considering spherical entangling regions. As entanglement entropy also includes divergences, we employ the Kounterterms scheme to extract the physically relevant quantities. In the case of three-dimensional CFTs dual to Einstein gravity, we show that the finite part is isolated and can be written in terms of the Willmore energy, providing an upper bound based on its properties. We extend this remarkable result to arbitrary CFTs under consideration. Besides, we show the validity of the Kounterterms scheme for general quadratic curvature gravity, extracting the type A, type B anomalies of the theory in even dimensions and the sphere free energy in odd ones.

==> text/abbreviations.tex <==
% First parameter can be changed eg to "Glossary" or something.
% Second parameter is the max length of bold terms.
\begin{mclistof}{List of Abbreviations}{3.2cm}

\item[1-D, 2-D] One- or two-dimensional, referring in this thesis to spatial dimensions in an image.

\item[Otter] One of the finest of water mammals.

\item[Hedgehog] Quite a nice prickly friend.

\end{mclistof} 


==> text/appA.tex <==
\chapter{Redefining the metric}\label{App:2}
%One strategy that has been sometimes used in the literature consists in performing a field redefinition of the form
%\begin{equation}
%g_{ab}\rightarrow g_{ab}+\alpha K_{ab}\, ,
%\end{equation}
%where $K_{ab}$ is a tensor formed from the curvature, such as $K_{ab}=a R_{ab}+b R g_{ab}$. However, one has to be careful with this type of field-redefinitions, since they involve the metric and its derivatives. It is easy to see that it is not correct to substitute directly in the action a field redefinition that involves derivatives. However, the change of variables can be made algebraic if one introduces first auxiliary variables.


Implementing a differential change of variables directly in the action can be problematic if one is not careful enough. In order to see this, let us consider the equations of motion of $\tilde g_{ab}$ ---defined so that $g_{ab}=\tilde g_{ab}+ K_{ab}$--- by computing the variation of the new action $\tilde S[\tilde g_{ab}]=S[g_{ab}]$:\footnote{Note that in the second term we used the chain law for the functional derivative, which is in general  given by
\begin{equation}
\frac{\delta S}{\delta \phi}\frac{\delta \phi}{\delta \psi}=\frac{\delta S}{\delta \phi}\frac{\partial \phi}{\partial \psi}-\partial_{a}\left(\frac{\delta S}{\delta \phi}\frac{\partial \phi}{\partial_{a}\psi}\right)+\ldots
\end{equation}
}

\begin{equation}\label{eq:badeq}
\frac{\delta \tilde S}{\delta \tilde g_{ab}}=\frac{\delta S}{\delta g_{ab}}+\frac{\delta S}{\delta g_{ef}}\frac{\delta K_{ef}}{\delta \tilde g_{ab}} \Bigg|_{g_{ab}=\tilde g_{ab}+K_{ab}}\, .
\end{equation}
Now, it is clear that we can always solve these equations if
\begin{equation}\label{eq:goodeq}
\frac{\delta S}{\delta g_{ab}} \Bigg|_{g_{ab}=\tilde g_{ab}+K_{ab}}=0\, .
\end{equation}
In other words, implementing the change of variables directly in the equations of the original theory produces an equation that solves the equations of $\tilde S$. However, the equations of $\tilde S$ contain more solutions. These additional solutions are spurious and appear as a consequence of increasing the number of derivatives in the action, so they should not be considered. 
A possible way to formalize this intuitive argument consists in introducing auxiliary field so that the redefinition of the metric becomes algebraic. Let us consider the following action
\begin{align}
S_{\chi}=\frac{1}{16\pi G}\int \diff^D\sqrt{|g|}\Big[&-2\Lambda+R+f\left(g^{ab}, \chi_{abcd}, \chi_{e_1,abcd},\chi_{e_1e_2,abcd},\ldots\right)\\ \notag&+\frac{\partial f}{\partial \chi_{abcd}}\left(R_{abcd}-\chi_{abcd}\right)+\frac{\partial f}{\partial \chi_{e_1,abcd}}\left(\nabla_{e_1}R_{abcd}-\chi_{e_1,abcd}\right)\\ \notag &+\frac{\partial f}{\partial \chi_{e_1e_2,abcd}}\left(\nabla_{e_1}\nabla_{e_2}R_{abcd}-\chi_{e_1e_2,abcd}\right)+\ldots\Big]\, ,
\end{align}
where we have introduced some auxiliary fields $\chi_{abcd}$, $\chi_{e_{1},abcd}$, \ldots $\chi_{e_{1}\ldots e_{n},abcd}$. Let us convince ourselves that this action is equivalent to \req{eq:generalhdg}. When we take the variation with respect to $\chi_{e_{1}\ldots e_{i},abcd}$, we get
\begin{equation}
\sum_{j=0}\frac{\partial^2 f}{\partial\chi_{e_1\ldots e_i,abcd} \partial \chi_{a_1\ldots a_j,ghmn}}\left(\nabla_{a_1}\ldots\nabla_{a_j}R_{ghmn}-\chi_{a_1\ldots a_j,ghmn}\right)=0\, .
\end{equation}
In this way, we get a system of algebraic equations for the variables $\chi_{e_{1}\ldots e_{i},abcd}$ that always has the following solution
\begin{eqnarray}
\label{eq:solchi}
\chi_{abcd}&=&R_{abcd}\, ,\\
\chi_{e_1,abcd}&=&\nabla_{e_1}R_{abcd}\, ,\\
\chi_{e_1 e_2,abcd}&=&\nabla_{e_1}\nabla_{e_2}R_{abcd}\, ,\\
&\ldots&
\end{eqnarray}
This is the unique solution if the matrix of the system is invertible, and this is the expected case if $f$ is general. When we plug this solution back in the action we recover \req{eq:generalhdg} (with explicit Einstein-Hilbert and cosmological constant terms), so that both formulations are equivalent. 

Now let us perform the following redefinition of the metric in $S_{\chi}$:
\begin{equation}
g_{ab}= \tilde g_{ab}+\alpha K_{ab}\, ,\quad\text{where}\,\,\, K_{ab}=K_{ab}\left(\tilde g^{ef}, \chi_{efcd}, \chi_{a_1,efcd},\ldots\right)\, ,
\end{equation}
this is, $K_{ab}$ is a symmetric tensor formed from contractions of the $\chi$ variables and the metric, but it contains no derivatives of any field. In this way, the change of variables is algebraic and can be directly implemented in the action. We therefore get
\begin{equation}
\tilde{S}_{\chi}\left[\tilde{g}_{ab}, \chi\right]=S_{\chi}\left[\tilde{g}_{ab}+\alpha K_{ab}, \chi\right]\, ,
\end{equation}
where, for simplicity, we are collectively denoting all auxiliary variables by $\chi$.  Now, both actions are equivalent and so are the field equations:
\begin{eqnarray}
\label{eq:eqmetric}
\frac{\delta \tilde{S}_{\chi}}{\delta\tilde g_{ab}}&=&\frac{\delta S_{\chi}}{\delta g_{ab}}\bigg|_{g_{ab}= \tilde g_{ab}+\alpha K_{ab}}\, ,\\
\label{eq:eqchi}
\frac{\delta \tilde{S}_{\chi}}{\delta\chi}&=&\frac{\delta {S}_{\chi}}{\delta\chi}+\alpha \frac{\delta {S}_{\chi}}{\delta g_{ab}}\frac{\delta K_{ab}}{\delta\chi}\bigg|_{g_{ab}= \tilde g_{ab}+\alpha K_{ab}}\, .
\end{eqnarray}
Using the first equation into the second one, we see that the equations for the auxiliary variables become $\delta S_{\chi}/\delta\chi=0$, which of course have the same solution as before \req{eq:solchi}. When we take that into account, $K_{ab}$ becomes a tensor constructed from the curvature of the original metric $g_{ab}$, so that we get
\begin{equation}
g_{ab}= \tilde g_{ab}+\alpha K_{ab}\left(\tilde g^{ef}, R_{efcd}, \nabla_{\alpha_1}R_{efcd},\ldots\right)\, .
\end{equation}
%This is a complicated system from which we should obtain $g_{ab}$ as a function of $\tilde g_{ab}$.  Let us denote the solution by
%\begin{equation}
%g_{ab}= \tilde g_{ab}+\alpha \tilde K_{ab}\, .
%\end{equation}
Then, according to Eq.~\req{eq:eqmetric}, the equation for the metric $\tilde g_{ab}$ is simply obtained from the equation of $g_{ab}$ by substituting the change of variables:
\begin{equation}\label{eq:consistenteq}
\frac{\delta S_{\chi}}{\delta g_{ab}}\bigg|_{g_{ab}= \tilde g_{ab}+K_{ab}}=0\, .
\end{equation}
However, note that this is not the same as substituting \req{eq:solchi} in the action and taking the variation. This would yield instead
\begin{equation}\label{eq:fake}
\frac{\delta \tilde{S}_{\chi}\left[\tilde{g}_{ab}, \chi(\tilde g_{ab})\right]}{\delta\tilde g_{ab}}=\frac{\delta \tilde S_{\chi}}{\delta \tilde g_{ab}}+\frac{\delta \tilde{S}_{\chi}}{\delta\chi}\frac{\delta\chi}{\delta\tilde g_{ab}}=\frac{\delta S_{\chi}}{\delta g_{ab}}\bigg|_{g_{ab}= \tilde g_{ab}+\alpha K_{ab}}-\alpha \frac{\delta {S}_{\chi}}{\delta g_{ef}}\frac{\delta K_{ef}}{\delta\chi}\frac{\delta\chi}{\delta\tilde g_{ab}}\bigg|_{g_{ab}= \tilde g_{ab}+\alpha K_{ab}}\, .
\end{equation}
This equation is formally different to \req{eq:eqmetric} due to the second term, and it is equivalent to \req{eq:badeq}. The second term appears because the auxiliary variables $\chi(\tilde g_{\mu\nu})$ do not solve the equation $\delta \tilde{S}_{\chi}/\delta\chi=0$, but $\delta {S}_{\chi}/\delta\chi=0$. However, we must solve $\delta \tilde{S}_{\chi}/\delta\chi=0$ in order to get a solution of $\tilde{S}_{\chi}\left[\tilde{g}_{ab}, \chi\right]$, and according to \req{eq:eqchi} this would only happen if $(\delta {S}_{\chi}/\delta g_{ab}) (\partial K_{ab}/\partial\chi)=0$, so that the only consistent solutions of \req{eq:fake} are those which satisfy \req{eq:consistenteq}. 
This explains why the only solutions of \req{eq:badeq} we should consider are the ones satisfying 
\req{eq:goodeq}. 

\chapter{$W^n \nabla W\nabla W$ terms on SSS backgrounds} \label{apricot}
In this appendix we show that \req{eq:Inv3} holds. In order to do that, it is convenient to carry out the following change or radial coordinate in the SSS ansatz \req{SSS}:
\begin{equation}
\diff \tilde{r}^2=\frac{\diff r^2}{r^2 f(r)}\, .
\end{equation}
In these coordinates, the SSS metric reads
\begin{equation}
\diff s^2=r(\tilde{r})^2\bigg [ -\tilde{N}(\tilde{r})^2\tilde{f}(\tilde{r})\diff t^2+\diff \tilde{r}^2+\diff \Omega^2_{(D-2)} \bigg],
\end{equation}
where we denoted $\tilde{N}(\tilde{r})=N(r(\tilde{r}))$ and $\tilde{f}(\tilde{r})=f(r(\tilde{r}))$.

We use a tilde to denote tensor components in the new coordinates. Direct computation shows that the components of the Weyl tensor in these new coordinates have formally the same expression as in the original ones, namely,
\begin{equation}
\tensor{ \tilde{W}}{^{ab}_{cd}}=-2\tilde{\chi}(\tilde{r}) \frac{(D-3)}{(D-1)}\tensor{ \tilde{w}}{^{ab}_{cd}}\, ,
\end{equation}
where the tensorial structure $\tensor{ \tilde{w}}{^{ab}_{cd}}$ is given by
\begin{equation}
\tensor{ \tilde{w}}{^{ab}_{cd}}=2\tilde{\tau}^{[a}_{[c} \tilde{\rho}^{b]}_{d]}-\frac{2}{(D-2)} \left(\tilde{\tau}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}+\tilde{\rho}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]} \right)+\frac{2}{(D-2)(D-3)} \tilde{\sigma}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}\, ,
\end{equation}
and where $\tilde{\rho}_a^b$ denotes the projection onto our new radial coordinate $\tilde{r}$. If we define $\tilde{H}_a^b=\tilde{\tau}_a^b+\tilde{\rho}_a^b$, we may express $\tensor{ \tilde{w}}{^{ab}_{cd}}$ as
\begin{equation}
\tensor{ \tilde{w}}{^{ab}_{cd}}=\tilde{H}^{[a}_{[c} \tilde{H}^{b]}_{d]}-\frac{2}{(D-2)} \tilde{H}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}+\frac{2}{(D-2)(D-3)} \tilde{\sigma}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}\, .
\label{mywayw}
\end{equation}
Consequently, the covariant derivative of the Weyl tensor turns out to be
\begin{equation}
\left. \nabla_e \tensor{\tilde{W}}{^{ab}_{cd}}  \right|_{\rm SSS}=-2\frac{(D-3)}{(D-1)} \left[ \frac{\diff \tilde{\chi}}{\diff \tilde{r}} \delta_e^1 \tensor{ \tilde{w}}{^{ab}_{cd}}+\tilde{\chi}(\tilde{r}) \left. {\nabla}_e \tensor{ \tilde{w}}{^{ab}_{cd}} \right|_{\rm SSS} \right]\, ,
\end{equation}
where we are denoting the components of the covariant derivative of any tensor $T$ in our new coordinates as $\nabla_e \tilde{T}_{ab...}^{cd...}$. Hence we just need to work out $\left. {\nabla}_e \tensor{ \tilde{w}}{^{ab}_{cd}} \right|_{\rm SSS}$. Using \eqref{mywayw}, we find
\begin{equation}
\begin{split}
\nabla_e \tensor{ \tilde{w}}{^{ab}_{cd}}&=2 \nabla_e \tilde{H}^{[a}_{[c} \tilde{H}^{b]}_{d]}-\frac{2}{(D-2)} \nabla_e \tilde{H}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}\\&-\frac{2}{(D-2)} \nabla_e \tilde{\sigma}^{[a}_{[c} \tilde{H}^{b]}_{d]}+\frac{4}{(D-2)(D-3)} \nabla_e \tilde{\sigma}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}\, .
\end{split}
\end{equation}
Since $\nabla_e \tilde{H}_a^b+\nabla_e \tilde{\sigma}_a^b=0$, we just need to compute $\nabla_e \tilde{H}_a^b$. A straightforward calculation produces
\begin{equation}
\nabla_e \tilde{H}_a^b=\frac{1}{(r(\tilde{r}))^3}\frac{\diff r}{\diff \tilde{r}} \tilde{g}_{eg} \tilde{\sigma}_a^f \delta_1^b +\frac{1}{r(\tilde{r})}\frac{\diff r}{\diff \tilde{r}} (D-2) \tilde{\sigma}_e^b \delta_a^1\, .
\end{equation}
Using this, the covariant derivative of the Weyl tensor gives
\begin{align}
\label{cdwtab}
\left. \nabla_e \tensor{ \tilde{W}}{^{ab}_{cd}}  \right|_{\rm SSS}=&-2\frac{(D-3)}{(D-1)}  \frac{\diff \tilde{\chi}}{\diff\tilde{r}} \delta_e^1 \tensor{ \tilde{w}}{^{ab}_{cd}} -2\frac{(D-3)}{(D-1)} \tilde{\chi}(\tilde{r}) \frac{\diff r}{\diff\tilde{r}} \bigg[ \frac{2}{(r(\tilde{r}))^3} \tilde{g}_{ef} \tilde{\sigma}_{[c|}^{f} \delta_1^{[a} \tilde{H}_{| d]}^{b]}\\ \notag &+\frac{2(D-2)}{r(\tilde{r})} \tilde{\sigma}_e^{[a|} \delta_{[c}^1 \tilde{H}_{d]}^{|b]}-\frac{2 }{(D-2)(r(\tilde{r}))^3}\tilde{g}_{ef} \tilde{\sigma}_{[c|}^{f} \delta_1^{[a} \tilde{\sigma}_{| d]}^{b]}\\ \notag &-\frac{2}{r(\tilde{r})}\tilde{\sigma}_e^{[a|} \delta_{[c}^1 \tilde{\sigma}_{d]}^{|b]}  +\frac{2 }{(D-2)(r(\tilde{r}))^3}\tilde{g}_{ef} \tilde{\sigma}_{[c|}^{f} \delta_1^{[a} \tilde{H}_{| d]}^{b]}+\frac{2 }{r(\tilde{r})}\tilde{\sigma}_e^{[a|} \delta_{[c}^1 \tilde{H}_{d]}^{|b]}\\  \notag&-\frac{4}{(D-2)(D-3)(r(\tilde{r}))^3}\tilde{g}_{ef} \tilde{\sigma}_{[c|}^{f} \delta_1^{[a} \tilde{\sigma}_{| d]}^{b]}-\frac{4 }{(D-3)r(\tilde{r})}\tilde{\sigma}_e^{[a|} \delta_{[c}^1 \tilde{\sigma}_{d]}^{|b]} \bigg]\, .
\end{align}
Equipped with \eqref{cdwtab}, we may infer the general form of any invariant $\left. \mathcal{R}_2^{\{1,1\}} \right |_{\rm SSS}$ as defined in \req{eq:Inv2}. Since the $\left. \mathcal{R}_2^{\{1,1\}} \right |_{\rm SSS}$ are scalars, we can obtain them expressed in the original coordinates by performing all calculations in the new ones and then substituting any dependence on $\tilde{r}$ by the initial radial coordinate $r$.


We notice the following facts:
a) any $\left. \mathcal{R}_2^{\{1,1\}} \right |_{\rm SSS}$ will have three types of terms: those carrying  a factor $\tilde{\chi}^n \left (\diff \tilde{\chi}/\diff \tilde{r} \right)^2$,  those involving a factor $\tilde{\chi}^{n+1}(\diff \tilde{\chi}/\diff \tilde{r}) (\diff r/\diff\tilde{r})$ and a third type of terms with the common factor $\tilde{\chi}^{n+2}(\diff r/\diff \tilde{r}  )^2$; b) since $\tilde{r}$ is dimensionless, we infer that the first type of terms is not weighted by any power of $r$, the second type is accompanied by $r^{-1}$ and the third type, by $r^{-2}$. An additional overall factor of $r^{-2}$ is required by dimensional analysis.
Using these observations, it follows that
\begin{equation}
\left. \mathcal{R}_2^{\{1,1\}} \right |_{\rm SSS}=\frac{\tilde{\chi}^n(\tilde{r})}{r(\tilde{r})^2}\bigg[ c_1 \left (\frac{\diff \tilde{\chi}}{\diff \tilde{r}} \right)^2+c_2  \frac{\diff \tilde{\chi}}{\diff\tilde{r}} \frac{\diff r}{\diff\tilde{r}} \frac{\tilde{\chi}(\tilde{r})}{r(\tilde{r})}+c_3  \left ( \frac{\tilde{\chi}(\tilde{r})}{r(\tilde{r})} \right )^2 \left( \frac{\diff r}{\diff \tilde{r}}  \right)^2\bigg]\, ,
\end{equation}
for some constants $c_1$, $c_2$, $c_3$ which will depend on the specific term.
Taking into account that $\diff \tilde{r}/\diff r =1/ (r \sqrt{f(r)})$
%\begin{equation}
%\frac{d \tilde{r}}{dr}=\frac{1}{r\sqrt{f(r)}},
%\end{equation}
we finally find
\begin{equation}
\left. \mathcal{R}_2^{\{1,1\}} \right |_{\rm SSS}=\chi^n f(r)\left ( c_1  (\chi ')^2+c_2\frac{\chi \chi'}{r}+c_3 \frac{\chi^2}{r^2} \right ),
\end{equation}
where $\chi'=\diff \chi/\diff r$.

\chapter{Mutual information regularization of EE in the EMI model}\label{EMIMIregu}
In Section \ref{secemi} we computed $F$ numerically for many kinds of entangling regions in the EMI model. In order to do so, we introduced a small regulator $\delta$ along an auxiliary extra dimension, evaluated $F^{\rm \ssc EMI}(A)$ as a function of $\delta$ and then extracted the $\delta \rightarrow 0$ limit. However, as we explained in Section \ref{elipsq} there is an alternative way of regularizing EE that makes use of the MI of concentric regions and which yields converging results in the lattice. In this appendix we explore this alternative method for the EMI model in the case of elliptic entangling regions for the two geometric setups explained in Section \ref{elipsq}, namely: fixing a constant $\varepsilon$, and forcing the concentric regions to be ellipses. This will allow us to test to what extent we may expect both methods to differ in general when the size of the entangling regions cannot be considered to be extremely larger than the separation between the auxiliary regions ---which is always the case in the lattice. We will also verify the convergence of both methods between themselves and with the $\delta$ method used in the main text.

In the three-dimensional EMI model, the mutual information between two regions $A,B$ in a fixed time slice is given by
\begin{equation}\label{emimi}
I^{\rm \ssc EMI}(A,B)=-2\kappa_{(3)}\int_{\partial A}\diff\mathbf{r}_A\int_{\partial B}\diff\mathbf{r}_B\, \frac{\mathbf{n}_A\cdot\mathbf{n}_B}{\abs{\mathbf{r}_A-\mathbf{r}_B}^{2}}\, ,
\end{equation}
where the normal vectors are defined outwards to each region, respectively. This formula is manifestly non-divergent, as $\mathbf{r}_A$ and $\mathbf{r}_B$ correspond now to different regions. For regions $A,B$ parametrized by $[x_{A,B}(t),y_{A,B}(t)]$ we have
\begin{equation}\label{emimi}
I^{\rm \ssc EMI}(A,B)=-2\kappa_{(3)}\int_{\partial A}\diff t_A\int_{\partial B}\diff t_B\, \frac{ \dot y_A(t_A) \dot y_B(t_B) + \dot x_A(t_A) \dot x_B(t_B)  }{  (x_A(t_A)-x_B(t_B))^2+(y_A(t_A)-y_B(t_B))^2}\, .
\end{equation}


Applied to the setup required for regularizing the EE, as in \req{annulii}, we need to evaluate the mutual information $I^{\rm \ssc EMI}(A^+,A^-)$, which involves integrals over $\partial A^+=\partial \overline{A^+}$ and $\partial A^-$. Using the EE formula for the EMI model, \req{emiee}, it is easy to see that in $I^{\rm \ssc EMI}(A^+,A^-)$ the contributions from $\see^{\rm \ssc EMI}(\overline{A^+})$ and $\see^{\rm \ssc EMI}(A^-)$ cancel with the terms in $\see^{\rm \ssc EMI}(\overline{A^+ \cup A^-})$ which involve performing both integrals over  $\partial A^+$ or both integrals over $\partial A^-$. The only terms which survive are the ones which involve one integral over $\partial A^+$ and the other one over $\partial A^-$, in agreement with \req{emimi}. 


 
 \begin{figure}[t!] \centering
	\includegraphics[scale=0.7]{fifi.pdf}
	\caption{ \textsf{We plot $F_{(e)}^{\rm \ssc EMI}/F_0^{\rm \ssc EMI}$ for different values of the eccentricity $e= 0,\sqrt{3}/2,2\sqrt{2}/3,\sqrt{15}/4,2\sqrt{6}/5$ using the expressions \req{ik130emi} (purple dots) and \req{ik13emi} (blue diamonds). In the case of  \req{ik130emi}, we fix $\varepsilon=5$ and plot the results as a function of the semi-minor axis $b$. In the case of \req{ik13emi} we fix $b_2=b_1+7$ and plot the results as a function of $b=(b_1+b_2)/2$ as well. The straight lines correspond to the exact values obtained using the $\delta$ method, which can be also reproduced using \req{ik130emi} or \req{ik13emi} for sufficiently large values of $b$.}}
	\label{ref44}
\end{figure}
 

%\subsection{Constant $\varepsilon$}
%The relevant formulas for the two relevant cases, 
In the case in which we keep $\varepsilon$ constant for all points of the ellipse boundary, the relevant formula is
 \begin{equation}\label{ik130emi}
 F^{\rm \ssc EMI}_{(e)}=-\frac{1}{2}\left[  I^{\rm \ssc EMI}({\rm pseudoellipse }_{i},{\rm pseudoellipse}_{o})-k_{{\rm \ssc EMI}}^{(3)} \frac{4 a E[e^2]}{\varepsilon}\right]\, ,
 \end{equation}  
where the parametrization of the pseudoellipses appears in \req{rio} and $k_{{\rm \ssc EMI}}^{(3)}$ is defined in \req{kemi}. On the other hand, if we force the auxiliary regions to be ellipses, the relevant formula reads
 \begin{equation}\label{ik13emi}
 F^{\rm \ssc EMI}_{(e)}=-\frac{1}{2}\left[  I^{{\rm \ssc EMI}}({\rm ellipse }_{2},{\rm ellipse}_{1})-k_{{\rm \ssc EMI}}^{(3)} \int_0^{\frac{\pi}{2}} \diff t \frac{2(a_1+a_2)\sqrt{1-e^2 \cos^2 t} }{\varepsilon(t)}\right]\, ,
 \end{equation} 
where $a=(a_1+a_2)/2$, $b=(b_1+b_2)/2$ and the formula for $\varepsilon(t)$ appears in  \req{epis}.

As a first check, we have verified that both \req{ik130emi} and \req{ik13emi} produce results essentially identical to the ones obtained using the $\delta$ method for sufficiently large values of $b/\varepsilon$ ---\eg $b/\varepsilon \sim 100$ yields excellent results in all cases. On the other hand, practical limitations force us to consider smaller values of such a quotient when performing calculations in the lattice ($b/\varepsilon \sim 10$). In Fig.\,\ref{ref44} we have plotted the results achieved using both methods for values of $b$ similar to the ones considered in our lattice calculations in Section \ref{elipsq}. As we can see, in both cases the results tend to underestimate considerably the actual ones ---this underestimation tends to be greater as the eccentricity grows. Importantly, we observe that the pseudoellipses method makes a better job in approximating the actual results than the variable-$\varepsilon$ one. The difference between both methods becomes rather considerable for greater values of the eccentricity. For each eccentricity and each value of $b$, we can observe what is the factor we need to multiply the corresponding EMI result by in order to obtain the exact answer $F_{(e)}^{\rm \ssc EMI}$. We use such factors in Section \ref{elipsq} to correct the lattice results obtained for the corresponding values of $b/\delta$.


 






%\section{Comments on the isoperimetric inequality} \comment{this appendix should probably  be removed in the end}
%The main goal of this paper has been to test whether or not the disk is a global minimum of $F^{\rm \ssc EMI}$. Naturally, there is a well-known, simple, geometric functional for which we know this to be the case. This is given by the combination 
%\begin{equation}
%\mathcal{R}(A) \equiv  \frac{ \text{perimeter}(\partial A)^2}{4\pi \cdot \text{area}(A)}\, ,
%\end{equation}
%which satisfies the isoperimetric inequality,
%\begin{equation}\label{isopp}
%\mathcal{R} \geq 1\, , \quad  \text{with} \quad \mathcal{R}=1 \Leftrightarrow  A = \text{disk}\, .
%\end{equation}
%As we will see, there seems to be an important degree of similarity between the behavior of $F^{\rm \ssc EMI}$ and the one of $\mathcal{R}$ for the various regions we consider.

%It is interesting to compare \req{fmeze0} with the analogous result for the purely geometric quantity satisfying the isoperimetric  inequality \req{isopp}. 
%For regions consisting of small deformations of the disk of the form defined by \req{fiy}, we have
%\begin{align}
%\frac{\mathrm{perimeter}(\partial A)}{2\pi R}&=1+\frac{\epsilon  }{\sqrt{\pi}} a_0^{(c)}+\frac{\epsilon^2}{4\pi}\sum_{\ell \geq 1} \ell^2 \left[ (a^{(c)}_{\ell})^2+(a^{(s)}_{\ell})^2 \right]+ \mathcal{O}(\epsilon^4)\, , \\
%\frac{\mathrm{area}(A)}{\pi R^2}&=1+ \frac{2\epsilon}{\sqrt{\pi}}a_0^{(c)}+\frac{\epsilon^2}{2\pi}\left[ \sum_{\ell \geq 1}[(a^{(c)}_{\ell})^2+ (a^{(s)}_{\ell})^2]+2 (a_0^{(c)})^2 \right]+ \mathcal{O}(\epsilon^4)\, ,
%\end{align}
%and from these expressions
%\begin{equation}\label{Rpert}
%\mathcal{R}=1+\frac{\epsilon^2}{2\pi}\sum_{\ell\geq 2} \left(\ell^2-1\right)\left[ (a^{(c)}_{\ell})^2+(a^{(s)}_{\ell})^2 \right]+\mathcal{O}(\epsilon^4)\, .
%\end{equation}
%Observe that dilatations ($\ell=0$) modify both the area and the perimeter already at leading order in $\epsilon$, but they disappear from the combination $\mathcal{R}$, which is quadratic in the deformation. Again, the coefficient of this leading term is positive, as expected from \req{isopp}. 

%As we can see, there is a high degree of similarity between $F$ and $\mathcal{R}$ for small perturbations of the disk. They are both minimized by the disk region,  they both remain unchanged by $\ell=0,1$ deformations, and they include the $ \left(\ell^2-1\right)\left[ (a^{(c)}_{\ell})^2+(a^{(s)}_{\ell})^2 \right]$ combination. 

%On the other hand, they differ by the fact that $F$ depends on a theory-dependent coefficient, $C_{\ssc T}$, and by an extra $\ell$ which appears in the shape-dependent sum. Besides, $\mathcal{R}$ fails to satisfy some of the properties that a good $F$ ---\ie a good entanglement entropy universal term--- \comment{blah blah, strong superadditivity, clustering, etc.}

%As mentioned earlier, the purely geometric quantity $\mathcal{R}$ defined in \req{isopp} satisfies a property analogous to the one we would like to test for $F$ ---\ie the isoperimetric inequality. Hence, we may wonder what  is the analogous result 

%\comment{the following should probably be removed later}\\
%For $\mathcal{R}|_{\rm ellipse}$ as $e\rightarrow 1$ we have
%\begin{align}
%\mathcal{R}|_{\rm ellipse} =\frac{4 E[e^2]^2}{ \pi^2 \sqrt{1-e^2}}  \overset{e\rightarrow 1}{\simeq} \frac{4}{\pi^2 \sqrt{2} \sqrt{1-e}} \left[1+\frac{(e-1)}{4}[3+4\log \left(\frac{1-e}{8} \right)]+\mathcal{O}(e-1)^2 \right]\, .
%\end{align}
%Hence, we observe that the functional dependence on $(e-1)$ is the same as for $F|_{\rm ellipse}$ at leading order. Observe that a proper comparison of both quantities requires normalizing $F|_{\rm ellipse}$ by the disk result, $F_0$, so that both $F|_{\rm ellipse}/F_0$ and $\mathcal{R}$ tend to $1$ as $e\rightarrow 0$. While the coefficient of the leading $e\rightarrow 1$ term for $\mathcal{R}$ is just a fixed number, in the case of $F|_{\rm ellipse}/F_0$ this is controlled by $k^{(3)}/F_0$, which is a theory-dependent quantity. It is, nonetheless, a positive-definite number.
%\comment{until here}

%Funnily, 





==> text/appB.tex <==
\chapter{$W^n \nabla W\nabla W$ terms on SSS backgrounds} \label{apricot}
In this appendix we show that \req{eq:Inv3} holds. In order to do that, it is convenient to carry out the following change or radial coordinate in the SSS ansatz \req{SSS}:
\begin{equation}
\diff \tilde{r}^2=\frac{\diff r^2}{r^2 f(r)}\, .
\end{equation}
In these coordinates, the SSS metric reads
\begin{equation}
\diff s^2=r(\tilde{r})^2\bigg [ -\tilde{N}(\tilde{r})^2\tilde{f}(\tilde{r})\diff t^2+\diff \tilde{r}^2+\diff \Omega^2_{(D-2)} \bigg],
\end{equation}
where we denoted $\tilde{N}(\tilde{r})=N(r(\tilde{r}))$ and $\tilde{f}(\tilde{r})=f(r(\tilde{r}))$.

We use a tilde to denote tensor components in the new coordinates. Direct computation shows that the components of the Weyl tensor in these new coordinates have formally the same expression as in the original ones, namely,
\begin{equation}
\tensor{ \tilde{W}}{^{ab}_{cd}}=-2\tilde{\chi}(\tilde{r}) \frac{(D-3)}{(D-1)}\tensor{ \tilde{w}}{^{ab}_{cd}}\, ,
\end{equation}
where the tensorial structure $\tensor{ \tilde{w}}{^{ab}_{cd}}$ is given by
\begin{equation}
\tensor{ \tilde{w}}{^{ab}_{cd}}=2\tilde{\tau}^{[a}_{[c} \tilde{\rho}^{b]}_{d]}-\frac{2}{(D-2)} \left(\tilde{\tau}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}+\tilde{\rho}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]} \right)+\frac{2}{(D-2)(D-3)} \tilde{\sigma}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}\, ,
\end{equation}
and where $\tilde{\rho}_a^b$ denotes the projection onto our new radial coordinate $\tilde{r}$. If we define $\tilde{H}_a^b=\tilde{\tau}_a^b+\tilde{\rho}_a^b$, we may express $\tensor{ \tilde{w}}{^{ab}_{cd}}$ as
\begin{equation}
\tensor{ \tilde{w}}{^{ab}_{cd}}=\tilde{H}^{[a}_{[c} \tilde{H}^{b]}_{d]}-\frac{2}{(D-2)} \tilde{H}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}+\frac{2}{(D-2)(D-3)} \tilde{\sigma}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}\, .
\label{mywayw}
\end{equation}
Consequently, the covariant derivative of the Weyl tensor turns out to be
\begin{equation}
\left. \nabla_e \tensor{\tilde{W}}{^{ab}_{cd}}  \right|_{\rm SSS}=-2\frac{(D-3)}{(D-1)} \left[ \frac{\diff \tilde{\chi}}{\diff \tilde{r}} \delta_e^1 \tensor{ \tilde{w}}{^{ab}_{cd}}+\tilde{\chi}(\tilde{r}) \left. {\nabla}_e \tensor{ \tilde{w}}{^{ab}_{cd}} \right|_{\rm SSS} \right]\, ,
\end{equation}
where we are denoting the components of the covariant derivative of any tensor $T$ in our new coordinates as $\nabla_e \tilde{T}_{ab...}^{cd...}$. Hence we just need to work out $\left. {\nabla}_e \tensor{ \tilde{w}}{^{ab}_{cd}} \right|_{\rm SSS}$. Using \eqref{mywayw}, we find
\begin{equation}
\begin{split}
\nabla_e \tensor{ \tilde{w}}{^{ab}_{cd}}&=2 \nabla_e \tilde{H}^{[a}_{[c} \tilde{H}^{b]}_{d]}-\frac{2}{(D-2)} \nabla_e \tilde{H}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}\\&-\frac{2}{(D-2)} \nabla_e \tilde{\sigma}^{[a}_{[c} \tilde{H}^{b]}_{d]}+\frac{4}{(D-2)(D-3)} \nabla_e \tilde{\sigma}^{[a}_{[c} \tilde{\sigma}^{b]}_{d]}\, .
\end{split}
\end{equation}
Since $\nabla_e \tilde{H}_a^b+\nabla_e \tilde{\sigma}_a^b=0$, we just need to compute $\nabla_e \tilde{H}_a^b$. A straightforward calculation produces
\begin{equation}
\nabla_e \tilde{H}_a^b=\frac{1}{(r(\tilde{r}))^3}\frac{\diff r}{\diff \tilde{r}} \tilde{g}_{eg} \tilde{\sigma}_a^f \delta_1^b +\frac{1}{r(\tilde{r})}\frac{\diff r}{\diff \tilde{r}} (D-2) \tilde{\sigma}_e^b \delta_a^1\, .
\end{equation}
Using this, the covariant derivative of the Weyl tensor gives
\begin{align}
\label{cdwtab}
\left. \nabla_e \tensor{ \tilde{W}}{^{ab}_{cd}}  \right|_{\rm SSS}=&-2\frac{(D-3)}{(D-1)}  \frac{\diff \tilde{\chi}}{\diff\tilde{r}} \delta_e^1 \tensor{ \tilde{w}}{^{ab}_{cd}} -2\frac{(D-3)}{(D-1)} \tilde{\chi}(\tilde{r}) \frac{\diff r}{\diff\tilde{r}} \bigg[ \frac{2}{(r(\tilde{r}))^3} \tilde{g}_{ef} \tilde{\sigma}_{[c|}^{f} \delta_1^{[a} \tilde{H}_{| d]}^{b]}\\ \notag &+\frac{2(D-2)}{r(\tilde{r})} \tilde{\sigma}_e^{[a|} \delta_{[c}^1 \tilde{H}_{d]}^{|b]}-\frac{2 }{(D-2)(r(\tilde{r}))^3}\tilde{g}_{ef} \tilde{\sigma}_{[c|}^{f} \delta_1^{[a} \tilde{\sigma}_{| d]}^{b]}\\ \notag &-\frac{2}{r(\tilde{r})}\tilde{\sigma}_e^{[a|} \delta_{[c}^1 \tilde{\sigma}_{d]}^{|b]}  +\frac{2 }{(D-2)(r(\tilde{r}))^3}\tilde{g}_{ef} \tilde{\sigma}_{[c|}^{f} \delta_1^{[a} \tilde{H}_{| d]}^{b]}+\frac{2 }{r(\tilde{r})}\tilde{\sigma}_e^{[a|} \delta_{[c}^1 \tilde{H}_{d]}^{|b]}\\  \notag&-\frac{4}{(D-2)(D-3)(r(\tilde{r}))^3}\tilde{g}_{ef} \tilde{\sigma}_{[c|}^{f} \delta_1^{[a} \tilde{\sigma}_{| d]}^{b]}-\frac{4 }{(D-3)r(\tilde{r})}\tilde{\sigma}_e^{[a|} \delta_{[c}^1 \tilde{\sigma}_{d]}^{|b]} \bigg]\, .
\end{align}
Equipped with \eqref{cdwtab}, we may infer the general form of any invariant $\left. \mathcal{R}_2^{\{1,1\}} \right |_{\rm SSS}$ as defined in \req{eq:Inv2}. Since the $\left. \mathcal{R}_2^{\{1,1\}} \right |_{\rm SSS}$ are scalars, we can obtain them expressed in the original coordinates by performing all calculations in the new ones and then substituting any dependence on $\tilde{r}$ by the initial radial coordinate $r$.


We notice the following facts:
a) any $\left. \mathcal{R}_2^{\{1,1\}} \right |_{\rm SSS}$ will have three types of terms: those carrying  a factor $\tilde{\chi}^n \left (\diff \tilde{\chi}/\diff \tilde{r} \right)^2$,  those involving a factor $\tilde{\chi}^{n+1}(\diff \tilde{\chi}/\diff \tilde{r}) (\diff r/\diff\tilde{r})$ and a third type of terms with the common factor $\tilde{\chi}^{n+2}(\diff r/\diff \tilde{r}  )^2$; b) since $\tilde{r}$ is dimensionless, we infer that the first type of terms is not weighted by any power of $r$, the second type is accompanied by $r^{-1}$ and the third type, by $r^{-2}$. An additional overall factor of $r^{-2}$ is required by dimensional analysis.
Using these observations, it follows that
\begin{equation}
\left. \mathcal{R}_2^{\{1,1\}} \right |_{\rm SSS}=\frac{\tilde{\chi}^n(\tilde{r})}{r(\tilde{r})^2}\bigg[ c_1 \left (\frac{\diff \tilde{\chi}}{\diff \tilde{r}} \right)^2+c_2  \frac{\diff \tilde{\chi}}{\diff\tilde{r}} \frac{\diff r}{\diff\tilde{r}} \frac{\tilde{\chi}(\tilde{r})}{r(\tilde{r})}+c_3  \left ( \frac{\tilde{\chi}(\tilde{r})}{r(\tilde{r})} \right )^2 \left( \frac{\diff r}{\diff \tilde{r}}  \right)^2\bigg]\, ,
\end{equation}
for some constants $c_1$, $c_2$, $c_3$ which will depend on the specific term.
Taking into account that $\diff \tilde{r}/\diff r =1/ (r \sqrt{f(r)})$
%\begin{equation}
%\frac{d \tilde{r}}{dr}=\frac{1}{r\sqrt{f(r)}},
%\end{equation}
we finally find
\begin{equation}
\left. \mathcal{R}_2^{\{1,1\}} \right |_{\rm SSS}=\chi^n f(r)\left ( c_1  (\chi ')^2+c_2\frac{\chi \chi'}{r}+c_3 \frac{\chi^2}{r^2} \right ),
\end{equation}
where $\chi'=\diff \chi/\diff r$.



==> text/appX.tex <==
\section{Mutual information regularization of EE in the EMI model}\label{EMIMIregu}
In Section \ref{secemi} we computed $F$ numerically for many kinds of entangling regions in the EMI model. In order to do so, we introduced a small regulator $\delta$ along an auxiliary extra dimension, evaluated $F^{\rm \ssc EMI}(A)$ as a function of $\delta$ and then extracted the $\delta \rightarrow 0$ limit. However, as we explained in Section \ref{elipsq} there is an alternative way of regularizing EE that makes use of the MI of concentric regions and which yields converging results in the lattice. In this appendix we explore this alternative method for the EMI model in the case of elliptic entangling regions for the two geometric setups explained in Section \ref{elipsq}, namely: fixing a constant $\varepsilon$, and forcing the concentric regions to be ellipses. This will allow us to test to what extent we may expect both methods to differ in general when the size of the entangling regions cannot be considered to be extremely larger than the separation between the auxiliary regions ---which is always the case in the lattice. We will also verify the convergence of both methods between themselves and with the $\delta$ method used in the main text.

In the three-dimensional EMI model, the mutual information between two regions $A,B$ in a fixed time slice is given by
\begin{equation}\label{emimi}
I^{\rm \ssc EMI}(A,B)=-2\kappa_{(3)}\int_{\partial A}\diff\mathbf{r}_A\int_{\partial B}\diff\mathbf{r}_B\, \frac{\mathbf{n}_A\cdot\mathbf{n}_B}{\abs{\mathbf{r}_A-\mathbf{r}_B}^{2}}\, ,
\end{equation}
where the normal vectors are defined outwards to each region, respectively. This formula is manifestly non-divergent, as $\mathbf{r}_A$ and $\mathbf{r}_B$ correspond now to different regions. For regions $A,B$ parametrized by $[x_{A,B}(t),y_{A,B}(t)]$ we have
\begin{equation}\label{emimi}
I^{\rm \ssc EMI}(A,B)=-2\kappa_{(3)}\int_{\partial A}\diff t_A\int_{\partial B}\diff t_B\, \frac{ \dot y_A(t_A) \dot y_B(t_B) + \dot x_A(t_A) \dot x_B(t_B)  }{  (x_A(t_A)-x_B(t_B))^2+(y_A(t_A)-y_B(t_B))^2}\, .
\end{equation}


Applied to the setup required for regularizing the EE, as in \req{annulii}, we need to evaluate the mutual information $I^{\rm \ssc EMI}(A^+,A^-)$, which involves integrals over $\partial A^+=\partial \overline{A^+}$ and $\partial A^-$. Using the EE formula for the EMI model, \req{emiee}, it is easy to see that in $I^{\rm \ssc EMI}(A^+,A^-)$ the contributions from $\see^{\rm \ssc EMI}(\overline{A^+})$ and $\see^{\rm \ssc EMI}(A^-)$ cancel with the terms in $\see^{\rm \ssc EMI}(\overline{A^+ \cup A^-})$ which involve performing both integrals over  $\partial A^+$ or both integrals over $\partial A^-$. The only terms which survive are the ones which involve one integral over $\partial A^+$ and the other one over $\partial A^-$, in agreement with \req{emimi}. 


 
 \begin{figure}[t!] \centering
	\includegraphics[scale=0.7]{fifi.pdf}
	\caption{ \textsf{We plot $F_{(e)}^{\rm \ssc EMI}/F_0^{\rm \ssc EMI}$ for different values of the eccentricity $e= 0,\sqrt{3}/2,2\sqrt{2}/3,\sqrt{15}/4,2\sqrt{6}/5$ using the expressions \req{ik130emi} (purple dots) and \req{ik13emi} (blue diamonds). In the case of  \req{ik130emi}, we fix $\varepsilon=5$ and plot the results as a function of the semi-minor axis $b$. In the case of \req{ik13emi} we fix $b_2=b_1+7$ and plot the results as a function of $b=(b_1+b_2)/2$ as well. The straight lines correspond to the exact values obtained using the $\delta$ method, which can be also reproduced using \req{ik130emi} or \req{ik13emi} for sufficiently large values of $b$.}}
	\label{ref44}
\end{figure}
 

%\subsection{Constant $\varepsilon$}
%The relevant formulas for the two relevant cases, 
In the case in which we keep $\varepsilon$ constant for all points of the ellipse boundary, the relevant formula is
 \begin{equation}\label{ik130emi}
 F^{\rm \ssc EMI}_{(e)}=-\frac{1}{2}\left[  I^{\rm \ssc EMI}({\rm pseudoellipse }_{i},{\rm pseudoellipse}_{o})-k_{{\rm \ssc EMI}}^{(3)} \frac{4 a E[e^2]}{\varepsilon}\right]\, ,
 \end{equation}  
where the parametrization of the pseudoellipses appears in \req{rio} and $k_{{\rm \ssc EMI}}^{(3)}$ is defined in \req{kemi}. On the other hand, if we force the auxiliary regions to be ellipses, the relevant formula reads
 \begin{equation}\label{ik13emi}
 F^{\rm \ssc EMI}_{(e)}=-\frac{1}{2}\left[  I^{{\rm \ssc EMI}}({\rm ellipse }_{2},{\rm ellipse}_{1})-k_{{\rm \ssc EMI}}^{(3)} \int_0^{\frac{\pi}{2}} \diff t \frac{2(a_1+a_2)\sqrt{1-e^2 \cos^2 t} }{\varepsilon(t)}\right]\, ,
 \end{equation} 
where $a=(a_1+a_2)/2$, $b=(b_1+b_2)/2$ and the formula for $\varepsilon(t)$ appears in  \req{epis}.

As a first check, we have verified that both \req{ik130emi} and \req{ik13emi} produce results essentially identical to the ones obtained using the $\delta$ method for sufficiently large values of $b/\varepsilon$ ---\eg $b/\varepsilon \sim 100$ yields excellent results in all cases. On the other hand, practical limitations force us to consider smaller values of such a quotient when performing calculations in the lattice ($b/\varepsilon \sim 10$). In Fig.\,\ref{ref44} we have plotted the results achieved using both methods for values of $b$ similar to the ones considered in our lattice calculations in Section \ref{elipsq}. As we can see, in both cases the results tend to underestimate considerably the actual ones ---this underestimation tends to be greater as the eccentricity grows. Importantly, we observe that the pseudoellipses method makes a better job in approximating the actual results than the variable-$\varepsilon$ one. The difference between both methods becomes rather considerable for greater values of the eccentricity. For each eccentricity and each value of $b$, we can observe what is the factor we need to multiply the corresponding EMI result by in order to obtain the exact answer $F_{(e)}^{\rm \ssc EMI}$. We use such factors in Section \ref{elipsq} to correct the lattice results obtained for the corresponding values of $b/\delta$.


 






%\section{Comments on the isoperimetric inequality} \comment{this appendix should probably  be removed in the end}
%The main goal of this paper has been to test whether or not the disk is a global minimum of $F^{\rm \ssc EMI}$. Naturally, there is a well-known, simple, geometric functional for which we know this to be the case. This is given by the combination 
%\begin{equation}
%\mathcal{R}(A) \equiv  \frac{ \text{perimeter}(\partial A)^2}{4\pi \cdot \text{area}(A)}\, ,
%\end{equation}
%which satisfies the isoperimetric inequality,
%\begin{equation}\label{isopp}
%\mathcal{R} \geq 1\, , \quad  \text{with} \quad \mathcal{R}=1 \Leftrightarrow  A = \text{disk}\, .
%\end{equation}
%As we will see, there seems to be an important degree of similarity between the behavior of $F^{\rm \ssc EMI}$ and the one of $\mathcal{R}$ for the various regions we consider.

%It is interesting to compare \req{fmeze0} with the analogous result for the purely geometric quantity satisfying the isoperimetric  inequality \req{isopp}. 
%For regions consisting of small deformations of the disk of the form defined by \req{fiy}, we have
%\begin{align}
%\frac{\mathrm{perimeter}(\partial A)}{2\pi R}&=1+\frac{\epsilon  }{\sqrt{\pi}} a_0^{(c)}+\frac{\epsilon^2}{4\pi}\sum_{\ell \geq 1} \ell^2 \left[ (a^{(c)}_{\ell})^2+(a^{(s)}_{\ell})^2 \right]+ \mathcal{O}(\epsilon^4)\, , \\
%\frac{\mathrm{area}(A)}{\pi R^2}&=1+ \frac{2\epsilon}{\sqrt{\pi}}a_0^{(c)}+\frac{\epsilon^2}{2\pi}\left[ \sum_{\ell \geq 1}[(a^{(c)}_{\ell})^2+ (a^{(s)}_{\ell})^2]+2 (a_0^{(c)})^2 \right]+ \mathcal{O}(\epsilon^4)\, ,
%\end{align}
%and from these expressions
%\begin{equation}\label{Rpert}
%\mathcal{R}=1+\frac{\epsilon^2}{2\pi}\sum_{\ell\geq 2} \left(\ell^2-1\right)\left[ (a^{(c)}_{\ell})^2+(a^{(s)}_{\ell})^2 \right]+\mathcal{O}(\epsilon^4)\, .
%\end{equation}
%Observe that dilatations ($\ell=0$) modify both the area and the perimeter already at leading order in $\epsilon$, but they disappear from the combination $\mathcal{R}$, which is quadratic in the deformation. Again, the coefficient of this leading term is positive, as expected from \req{isopp}. 

%As we can see, there is a high degree of similarity between $F$ and $\mathcal{R}$ for small perturbations of the disk. They are both minimized by the disk region,  they both remain unchanged by $\ell=0,1$ deformations, and they include the $ \left(\ell^2-1\right)\left[ (a^{(c)}_{\ell})^2+(a^{(s)}_{\ell})^2 \right]$ combination. 

%On the other hand, they differ by the fact that $F$ depends on a theory-dependent coefficient, $C_{\ssc T}$, and by an extra $\ell$ which appears in the shape-dependent sum. Besides, $\mathcal{R}$ fails to satisfy some of the properties that a good $F$ ---\ie a good entanglement entropy universal term--- \comment{blah blah, strong superadditivity, clustering, etc.}

%As mentioned earlier, the purely geometric quantity $\mathcal{R}$ defined in \req{isopp} satisfies a property analogous to the one we would like to test for $F$ ---\ie the isoperimetric inequality. Hence, we may wonder what  is the analogous result 

%\comment{the following should probably be removed later}\\
%For $\mathcal{R}|_{\rm ellipse}$ as $e\rightarrow 1$ we have
%\begin{align}
%\mathcal{R}|_{\rm ellipse} =\frac{4 E[e^2]^2}{ \pi^2 \sqrt{1-e^2}}  \overset{e\rightarrow 1}{\simeq} \frac{4}{\pi^2 \sqrt{2} \sqrt{1-e}} \left[1+\frac{(e-1)}{4}[3+4\log \left(\frac{1-e}{8} \right)]+\mathcal{O}(e-1)^2 \right]\, .
%\end{align}
%Hence, we observe that the functional dependence on $(e-1)$ is the same as for $F|_{\rm ellipse}$ at leading order. Observe that a proper comparison of both quantities requires normalizing $F|_{\rm ellipse}$ by the disk result, $F_0$, so that both $F|_{\rm ellipse}/F_0$ and $\mathcal{R}$ tend to $1$ as $e\rightarrow 0$. While the coefficient of the leading $e\rightarrow 1$ term for $\mathcal{R}$ is just a fixed number, in the case of $F|_{\rm ellipse}/F_0$ this is controlled by $k^{(3)}/F_0$, which is a theory-dependent quantity. It is, nonetheless, a positive-definite number.
%\comment{until here}

%Funnily, 


==> text/declaration.tex <==

\large I, Javier Moreno, hereby declare that this thesis, titled \textsl{Higher-Curvature Gravity and Entanglement Entropy} and the work presented in it is entirely my own. Where I have consulted the work of others, this is always clearly stated.\\

Date:\hfill Signature:

==> text/listofp.tex <==
The following articles were published by the candidate and his collaborators during the realization of the thesis: 
\begin{etaremune}

\item Pablo Bueno, Pablo A. Cano, R. A. Hennigar, Mengqi Lu, Javier Moreno, \textit{In preparation}

\item Pablo Bueno, Pablo A. Cano, Quim Llorens, Javier Moreno, Guido van der Welde\\
Aspects of three-dimensional higher curvatures gravities 
[22XX.XXXXX]. 

\item Pablo Bueno, Horacio Casini, Oscar Lasso Andino, Javier Moreno\\
 \textit{Disks globally maximize the entanglement entropy in 2+1 dimensions}\\
 \JHEP \textbf{10} (2021) 179 [\href{https://arxiv.org/abs/2107.12394}{2107.12394}]. 

\item Pablo Bueno, Pablo A. Cano, Javier Moreno, Guido van der Velde\\
 \textit{Regular black holes in three dimensions}\\
\PRD \textbf{104} (2021) L021501 [\href{https://arxiv.org/abs/2104.10172}{2104.10172}]

\item Giorgos Anastasiou, Ignacio J. Araya, Javier Moreno, Rodrigo Olea, David Rivera-Betancour\\
 \textit{Renormalized holographic entanglement entropy for Quadratic Curvature Gravity}\\
\PRD \textbf{104} (2021) 086003 [\href{https://arxiv.org/abs/2002.06111}{2102.11242}]

\item Giorgos Anastasiou, Javier Moreno, Rodrigo Olea, David Rivera-Betancour\\
 \textit{Shape dependence of renormalized holographic entanglement entropy}\\
 \JHEP \textbf{09} (2020) 173 [\href{https://arxiv.org/abs/2002.06111}{2002.06111}]

\item Pablo Bueno, Pablo A. Cano, Javier Moreno, \'Angel Murcia\\
 \textit{All higher-curvature gravities as Generalized quasi-topological gravities}\\
 \JHEP \textbf{11} (2019) 062 [\href{https://arxiv.org/abs/1906.00987}{1906.00987}]
 \end{etaremune}
